Flow optimization process in a transportation network

Numerous networks, such as transportation, distribution and delivery networks optimize their designs in order to increase efficiency and lower costs, improving the stability of its intended functions, etc. Networks that distribute goods, such as electricity, water, gas, telephone and data (Internet), or services as mail, railways and roads are examples of transportation networks. The optimal design fixes network architecture, including clustering, degree distribution, hierarchy, community structures and other structural metrics. These networks are specifically designed for efficient transportation, minimizing transit times and costs. All sorts of transportation networks face the same problem: traffic congestion among their channels. In this work we considered a transportation network model in which we optimize/minimize a cost function for the flux/current at each channel/link of the network. We performed simulations and an analytical study of this problem, focusing on the fraction of used channels and the flow distribution through these channels. Our results show that, after the initial transient, the fraction of used channels stays constant and, remarkably, this result does not depend on the lattice structure (2D, 3D, or long-range connections). For the case of high flow, all channels in the network are used. On the other hand, in the small flow limit, we observe a novel behavior that the fraction of used channels depends on the square root of the flow.

==> appendices.tex <==

\appendix*
\section{Mean field recurrence equations}

The integral recurrence equations of the current distributions on vertexes $\mathcal{Q}_t(j)$, on channels $\mathcal{P}_t(j)$ and the fraction of empty vertexes $B_t$ are given by 

\onecolumngrid
\begin{align}
\label{generalrec}
\mathcal{Q}_t(j) & = 2B_t \mathcal{P}_t(j) + \int_0^j \mathcal{P}_t(j)\mathcal{P}_t(j-J) dJ \\
\label{generalrec2}
\mathcal{P}_{t+1}(j) & = \frac{\mathcal{V}(j)}{2}\mathcal{Q}_t(j) + 2\int_0^\infty v(J)\mathcal{Q}_t(2j+J) dJ + 2 \int_0^j v(J)\mathcal{Q}_t(2j-J) dJ \\
B_{t+1} & = B_t^2+ \frac{1}{2}\int_0^\infty \mathcal{V}(j)\mathcal{Q}_t(j) dj
\end{align}
\twocolumngrid
\noindent where $\mathcal{V}(j)$ is two times the complementary cumulative distribution of critical currents distribution $v(j)$ defined by the channel costs, the $2$ factor is due the costs values degenerescence by two channels.

The set of equations above follow the current split rule on a bifurcation: (i) in time $t$, $\mathcal{Q}_t$ has two terms, the first one is the empty channel plus filled one by a current $j$ and the second term is the coalescence of two filled channels; (ii) next step ($t+1$) one random channel receives a current $j$ if this one is bellow the critical current defined by the $v(j)$ distribution, first term or one channel probability, otherwise the $j$ value will depend on the current split probability, second and third terms; (iii) finally the empty channel probability on the next step depends on two empty channels, first term, and one filled channel joins to a empty one, second term.


==> meanfield.tex <==
\section{Mean-Field approach}

For a infinite system one should considered a mean-field version of this model. For that case, the nodes are also organized by layers and each node has two outgoing channels but the channels are randomly selected in pairs from the next layer, suppressing local correlations and changing the systems dimension to 1 + $\infty$. The structure is composed by an infinite number of consecutive layers of nodes, through which the current passes only once, without any loops on the network. In our model this dynamics is equivalent to the multilayer structure.

The flow distribution in the first layer depends on the initial distribution $P(j,t=0)$ and in the second layer depends on previously layer, and consequently on the initial distribution as well, and so on for the next layers. For the case when t $\rightarrow \infty$ the stationary current distribution is independent of initial conditions, with exception for the initial average current.

% Estava em negrito o texto
Simulations were supported by a mean-field theory~\cite{Rui-Orahcio,Orahcio} which gives

\begin{equation}
 1 - B = 2\sqrt{\langle j\rangle},
\end{equation}
and
\begin{equation}
 P(j)=4e^{\frac{-2j}{\sqrt{\langle j\rangle}}} 
\end{equation}
for small $\langle j \rangle$, as it is shown in Fig~\ref{fig_P(j)s}. Our simulations demonstrate that these laws work also in 2D and 3D and for large $\langle j \rangle$, beyond the limits of the applicability of any MF theory.
% fim do texto que estava em negrito


The minimal cost condition (eqs.~\ref{flow1st} and~\ref{flow2nd}) imposes a conditional probability $\mathcal{F}(j|J,I_c)$ for the output current $j$ given an input flow $J$ and the minimum value $I_c$,

\begin{eqnarray}
\mathcal{F}(j|J,I_c)  & = &  \left[ \frac{1}{2}\delta(j) +\frac{1}{2}\delta(j-J)\right]\Theta(I_c-J)+\nonumber\\
 & & + \left[\frac{1}{2}\delta\left(j-\frac{J-I_c}{2}\right)\right. +\nonumber\\
 & & \left. +\frac{1}{2}\delta\left(j-\frac{J+I_c}{2}\right)\right]\Theta(J-I_c)
\label{deltas}
\end{eqnarray}
where $\delta(j)$ and $\Theta(j)$ are the delta and step distributions respectively.

Since $\mathcal{P}_t(j)$ and $\mathcal{Q}_t(j)$ are the current distributions on the channels and the vertexes respectively at discrete time $t$, we can write a set of recursive integral equations (see appendix) for these distributions and the empty channels probability $B_t$, straightly defined by the $\mathcal{P}_t(j)$ distribution
\begin{equation}
B_t = 1 - \int_0^\infty \mathcal{P}_t(j)dj.
\end{equation}

The cost distribution -- or the critical current distribution $v(I_c)$ -- is an important factor on the final form of the above distributions. We propose a simple shape for that distribution to perform the mean field approach,
\begin{equation}
v(I_c) = \frac{1}{\beta^2}\Theta(\beta-I_c)
\end{equation}
is the uniform case, where the critical flow are uniformly distributed on the net, therefore, $\beta$ is the maximum critical current found.

The solution of the recurrence equations set can be an exhaustive task even for computers, each point in the next distribution depends on the integration of thousand points in the previous distribution. But that set of equations allows some limit approaches for steady terms like the empty channel probability $B$ for small currents, the coefficient $\mathcal{P}(0)$ for the current channel distribution, still on the small current limit and the large current limit distribution.

On the small current limit, the uniform case gives a steady equation for the $B$ probability in the form
\begin{equation}
B(\langle j\rangle,\langle j^2\rangle_\mathcal{Q}) = 1-2\sqrt{\langle j\rangle - \frac{\langle j^2\rangle_\mathcal{Q}}{4}},
\end{equation}
where we choose $\beta=1$ and the $\langle\rangle$ denotes a moment performed by the $\mathcal{P}(j)$ distribution and the $\langle\rangle_\mathcal{Q}$ for the $\mathcal{Q}(j)$ one. The numerical integration of the \ref{generalrec} equations with $t_{max}=250$ time steps, allow us the strong assumption for the second moment $\langle j^2\rangle_\mathcal{Q}$, it decays to zero faster than the average current $\langle j\rangle$. So the probability of active channels is $1-B\sim\langle j\rangle ^{1/2}$ on this limit.

By an analog way, the steady coefficient $\mathcal{P}(0)$ can be evaluated with the \emph{posteriori} current distribution on the \ref{generalrec} equations,
\begin{equation}
\mathcal{P}(0) = 2(1+B)-4\frac{\langle j\rangle}{1-B}.
\end{equation}
Since $B\rightarrow 1$ for the small current limit and $1-B$ goes to zero slower than the average current, according the previous assumption, thus the steady coefficient $P(0)=~4$.

For the large currents limit $\langle j\rangle\geqslant\beta$, we can employ Laplace transform technique~\cite{ross} on recurrence equations~\ref{generalrec} and~\ref{generalrec2}. Since $\Pi(z)$ and $K(z)$ are the transforms for $\mathcal{P}(j)$ and $\mathcal{Q}(j)$ distributions respectively, the Laplace recurrence equations become 
\begin{equation}
\Pi_{t+1}(z) = \left[\frac{4}{\beta z}\sinh\left(\frac{\beta z}{4}\right) \Pi_t\left(\frac{z}{2} \right)\right]^2.
\label{largeite}
\end{equation}

If an initial distribution for channels is proposed, there will be a final form for the limit of infinite iterations on the above equation~\ref{largeite}. After $n$ iterations it can be able to invert analytically that equation an perform numerically the inset plot on figure~\ref{fig_P(j)}.

The shape of the above distribution is close to a normal one, but by evaluation of each moment generating function derivatives, equation~\ref{largeite}, on the $z\rightarrow 0$ limit, we conclude that the steady distribution has just three moments equal to the normal distribution ones: the mean, the variance and the third moment. Table~\ref{tab:moments} compares first five non null central moments between the steady distribution and the normal one.

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[ht]
\caption{\label{tab:moments} Top six non-null moments of normal (A) and the steady distribution for large currents from this paper (B). Variance $\sigma^2=\nicefrac{\beta^2}{12}$.}
\begin{tabular}{@{}lccccc@{}}
\hline
\textbf{Order}      & \textbf{2nd}        & \textbf{4th}                         & \textbf{6th}                            & \textbf{8th}                                   & \textbf{10th}                                       \\ \hline
\textbf{A}     & $\sigma^2$ & $3\sigma^4$                 & $15\sigma^6$                   & $105\sigma^6$                         & $945\sigma^6$                              \\
\textbf{B} & $\sigma^2$ & $\frac{99}{35}\sigma^4$ & $\frac{2745}{217}\sigma^6$ & $\frac{10409283}{137795}\sigma^8$ & $\frac{12298729365}{22129877}\sigma^{10}$ \\ \hline
\end{tabular}
\end{table}
 

